Automatic recognition and tagging of topologically different regimes in dynamical systems

Complex systems are commonly modeled using nonlinear dynamical systems. These models are often high-dimensional and chaotic. An important goal in studying physical systems through the lens of mathematical models is to determine when the system undergoes changes in qualitative behavior. A detailed description of the dynamics can be difficult or impossible to obtain for high-dimensional and chaotic systems. Therefore, a more sensible goal is to recognize and mark transitions of a system between qualitatively different regimes of behavior. In practice, one is interested in developing techniques for detection of such transitions from sparse observations, possibly contaminated by noise. In this paper we develop a framework to accurately tag different regimes of complex systems based on topological features. In particular, our framework works with a high degree of success in picking out a cyclically orbiting regime from a stationary equilibrium regime in high-dimensional stochastic dynamical systems.

==> commands.tex <==
%% mathcal
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calZ}{\mathcal{Z}}

%% Measure theory shortcuts
\newcommand{\nua}{\nu_{\alpha}}
\newcommand{\Fa}{F_{\alpha}}

%% Misc mathcal
\newcommand{\calCe}{\mathcal{C}_{\eps}}
\newcommand{\calMe}{\mathcal{M}_{\eps}}
\newcommand{\calMee}{\mathcal{M}_{\eps'}}
\newcommand{\calNe}{\mathcal{N}_{\eps}}
\newcommand{\calRe}{\mathcal{R}_{\eps}}
\newcommand{\calRee}{\mathcal{R}_{\eps'}}
\newcommand{\calSe}{\mathcal{S}_{\eps}}

%% mathbb
\newcommand{\E}{\mathbb{E}}
\newcommand{\nats}{\mathbb{N}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\ints}{\mathbb{Z}}

%% Greek
\newcommand{\eps}{\varepsilon}
\newcommand{\lam}{\lambda}
\newcommand{\hnu}{\hat{\nu}}

%% Misc math arrows 
\newcommand{\ra}{\rightarrow}
\newcommand{\rra}{\rightrightarrows}
\newcommand{\hookra}{\hookrightarrow}

%% Just plain misc
\newcommand{\ds}{\displaystyle} 
\newcommand{\etal}{{\em et al.}}
\newcommand{\cech}{\v{C}ech}
\newcommand{\holder}{H\"{o}lder }
\newcommand{\falpha}{f(\alpha)}
\newcommand{\henon}{H\'{e}non }

%% From ftp://ftp.ams.org/ams/doc/amsmath/short-math-guide.pdf
% \providecommand{\abs}[1]{\lvert#1\rvert}
\providecommand{\norm}[1]{\lVert#1\rVert}

%% from Latex wikibook
% New definition of square root:
% it renames \sqrt as \oldsqrt
% \let\oldsqrt\sqrt
% % it defines the new \sqrt in terms of the old one
% \def\sqrt{\mathpalette\DHLhksqrt}
% \def\DHLhksqrt#1#2{%
% \setbox0=\hbox{$#1\oldsqrt{#2\,}$}\dimen0=\ht0
% \advance\dimen0-0.2\ht0
% \setbox2=\hbox{\vrule height\ht0 depth -\dimen0}%
% {\box0\lower0.4pt\box2}}

%\newcommand{\cs3}{\frac{1}{3}\text{-Cantor set}}

%% This chokes when used with Beamer. ????
%\newcommand{\vect}[1]{\mathbf{#1}}   %{\boldsymbol{#1}}

%% hyphenation
\hyphenation{wave-let}

